Agentic Keyframe Search for Video Question Answering

Video question answering (VideoQA) enables machines to extract and comprehend key information from videos through natural language interaction, which is a critical step towards achieving intelligence. However, the demand for a thorough understanding of videos and high computational costs still limit the widespread applications of VideoQA. To address it, we propose Agentic Keyframe Search (AKeyS), a simple yet powerful algorithm for identifying keyframes in the VideoQA task. It can effectively distinguish key information from redundant, irrelevant content by leveraging modern language agents to direct classical search algorithms. Specifically, we first segment the video and organize it as a tree structure. Then, AKeyS uses a language agent to estimate heuristics and movement costs while dynamically expanding nodes. Finally, the agent determines if sufficient keyframes have been collected based on termination conditions and provides answers. Extensive experiments on the EgoSchema and NExT-QA datasets show that AKeyS outperforms all previous methods with the highest keyframe searching efficiency, which means it can accurately identify key information and conduct effective visual reasoning with minimal computational overhead. For example, on the EgoSchema subset, it achieves 1.8% higher accuracy while processing only 43.5% of the frames compared to VideoTree. We believe that AKeyS represents a significant step towards building intelligent agents for video understanding. The code is publicly available at https://github.com/fansunqi/AKeyS.

==> sec/8_limitations.tex <==
\section{Limitations and Future Work}
\label{sec:limitations}
The primary limitation of this work is the high financial cost associated on querying LLM APIs. While using open-source LLMs can help reduce expenses to some extent, it still does not eliminate the computational complexity involved. However, there is no free lunch in the world. Video question answering is a highly complex task that involves both temporal and spatial challenges. It requires the integration of large-scale neural networks with complex symbolic rules to effectively separate key information from redundant content. 

Looking ahead, we aim to introduce a suite of swift and lightweight video analysis tools and then develop novel algorithms to optimize the tool usage, moving towards building a more powerful video agent and improving the accuracy and efficiency of various video understanding tasks.
